Samples on Thin Ice: Re-Evaluating Adversarial Pruning of Neural Networks

Neural network pruning has shown to be an effective technique for reducing the network size, trading desirable properties like generalization and robustness to adversarial attacks for higher sparsity. Recent work has claimed that adversarial pruning methods can produce sparse networks while also preserving robustness to adversarial examples. In this work, we first re-evaluate three state-of-the-art adversarial pruning methods, showing that their robustness was indeed overestimated. We then compare pruned and dense versions of the same models, discovering that samples on thin ice, i.e., closer to the unpruned model's decision boundary, are typically misclassified after pruning. We conclude by discussing how this intuition may lead to designing more effective adversarial pruning methods in future work.

==> background.tex <==

% old sect.2 starts here
\section{Background on Pruning and Robustness}
Recently, pruning has become a widely employed compression technique \cite{blalock_what_2020}. Concurrently, Adversarial Machine Learning has established itself as a well-developed branch, offering a massive number of remarkable results for both defenses and attacks~\cite{biggio_wild_2018}. Studies on pruning and robustness have different origins in different periods of time, but then later team up amid the Deep Learning takeover. In fact, in the last years, several works have analyzed pruning's effect on robustness and proposed counteractions. This section aims to illustrate the basic concepts of neural network pruning and its extensions to produce sparse and robust models. 

\myparagraph{Pruning.} Pruning~\cite{lecun_optimal_1990,janowsky_pruning_1989}, from a standard perspective, can be regarded as the act of removing parameters (weights) or entire structures of a network in order to make it sparse while not jeopardizing performances. Parameters can either be pruned individually based on some heuristic (unstructured pruning, \cite{DBLP:journals/corr/HanPTD15}) or into structures such as filters (structured pruning, \cite{Hao_pruning_for_efficient}). The method on which to choose the parameters to prune defines instead whether the parameters, such as weights, are deemed unnecessary and can be pruned. Commonly used methods are the lowest weight-magnitude \cite{DBLP:journals/corr/HanPTD15}, and the lowest gradient-magnitude-based pruning \cite{nisp_yu}. The locality of pruning instead defines whether the weights or, in general, parameter removal has to be applied to a specific portion of the network (local pruning) or the entire network (global) \cite{blalock_what_2020}. Finally, the pruning pipeline defines how many times the network has to undergo the ``prune-finetune'' procedure to reach the final sparsity (either one-shot pruning or iterative pruning \cite{blalock_what_2020}) and in which stage of a learning process (pre, post or in-training). 

\myparagraph{Pruning and Robustness.} A modular pruning pipeline is based on the following steps: \textit{(i)} Pre-train a big model; \textit{(ii)} Prune the model according to some chosen method, locality, and criteria; \textit{(iii)} Fine-tune the model to make up for lost performances; \textit{(iv)} Stop or repeat the procedure of \textit{(ii)} and \textit{(iii)} iteratively. In its course, it is straightforward to augment the pipeline with robust objectives either when pre-training by using robust models, when pruning with a robustness-guided heuristic and, eventually, while fine-tuning, by doing it with a robust objective. 
\begin{equation}\label{eq:adv_train}
    \min _\theta \mathbb{E}_{(x, y) \sim \mathcal{D}}\left[\max _{\delta \in B(x, \varepsilon)} \mathcal{L}(\theta, x+\delta, y)\right]
\end{equation}
Equation~\ref{eq:adv_train} shows the Adversarial Training formulation as conceived by \cite{madry_towards_2019}, where $(x,y)\sim\mathcal{D}$ refers to the sampled training data and $B(x, \varepsilon)$ to the allowed set for the perturbation $\delta$ bounded by $\epsilon$. The goal of Equation~\ref{eq:adv_train} is to solve a min-max optimization problem, where the loss, denoted by $\mathcal{L}$,is minimized (outer problem) for its worst case (inner problem). Through this formulation, the expressed goal is to train the model to be robust to adversarial examples. It follows that this formulation can be integrated into most of the pruning pipeline steps, thus leading over the years to a great and diverse fashion of methods for obtaining sparse and robust networks.
Following also the contributions of \cite{wijayanto_robustness_2018, sehwag_towards_2019, dhillon_stochastic_2018, guo_sparse_2019, https://doi.org/10.48550/arxiv.1810.00208}, which are extensively discussed in Section~\ref{sect:related}, several methods blending pruning and robustness have achieved notable results. 

\myparagraph{ATMC.} The method proposed in \cite{gui_model_2019}, short for Adversarially Trained Model Compression, employs different compression pipelines (pruning, factorization and quantization) as constraints to a robust objective. 
\begin{equation}\label{eq:atmc}
    \resizebox{0.5\textwidth}{!}{$ 
    \begin{array}{ll}
     \min _{\boldsymbol{\theta}} & \sum_{(x, y) \in \mathcal{Z}} f^{\mathrm{adv}}(\boldsymbol{\theta} ; x, y) \\
     \text { s.t. } & \underbrace{\sum_{l=1}^L\left\|\boldsymbol{U}^{(l)}\right\|_0+\left\|\boldsymbol{V}^{(l)}\right\|_0+\left\|\boldsymbol{C}^{(l)}\right\|_0}_{\|\boldsymbol{\theta}\|_0} \leq k, \text { (sparsity) } \\
     & \boldsymbol{\theta} \in \mathcal{Q}_b:=\left\{\boldsymbol{\theta}:\left|\boldsymbol{U}^{(l)}\right|_0 \leq 2^b,\left|\boldsymbol{V}^{(l)}\right|_0 \leq 2^b,\left|\boldsymbol{C}^{(l)}\right|_0 \leq 2^b \forall l \in[L]\right\}, \text{(quantization)}
    \end{array}$}
\end{equation}
As Equation~\ref{eq:atmc} shows, the robust objective which minimizes the adversarial loss is subject to two constraints. The sparsity constraint, by decomposing the weight matrix as $\mathbf{W}=\mathbf{UV}+\mathbf{C}$ for the purpose of integrating every compression method (a factorization, where $\mathbf{C}$ is the sparse error \cite{neyshabur2014sparse}), requires them to have a total number of zeroed elements (denoted by $\|\cdot\|_0$) less than $k$. In the quantization constraint instead, the decomposed matrix is constrained to have a bounded number of different non-zero values depending on the representation bits \textit{$b$}. The notation $|\cdot|_0$ indeed, counts the number of different values diverse than 0 within the matrix. The robustness evaluation has been made with both PGD and FGSM attacks \cite{madry_towards_2019, goodfellow_explaining}.

\myparagraph{ADMM.} The framework proposed in \cite{ye_adversarial_2021}, is based on the alternating direction method of multipliers-based pruning (ADMM) \cite{Zhang_2018}. The basic idea is to solve a problem by decomposing smaller and simpler problems \cite{8186925_boyd}. The framework formulation of concurrent adversarial training and weight pruning is reported in Equation~\ref{eq:admm}.
\begin{equation}\label{eq:admm}
   \resizebox{0.5\textwidth}{!}{$\begin{array}{ll}
      \min _{\boldsymbol{\theta}_i} & \mathbb{E}_{( x, y) \sim \mathcal{D}}\left[\max _{ \delta \in \boldsymbol{\Delta}} L(\boldsymbol{\theta}, x+\delta, y)\right]+\sum_{i=1}^N g_i\left(\mathbf{z}_i\right), \\
      \text { s.t. } & \boldsymbol{\theta}_i=\mathbf{z}_i, i=1, \ldots, N .
      \end{array}$}
\end{equation}
Where $\theta_i$ are the weight parameters in each layer, and $g_i(\theta_i)$ is a function that can incorporate different pruning schemes based on the choice of the set $S_i$ defined as: 
\begin{equation}\label{eq:admm_g_function}
    \resizebox{0.2\textwidth}{!}{$
    g_i\left(\boldsymbol{\theta}_i\right)= \begin{cases}0 & \text { if } \boldsymbol{\theta}_i \in S_i \\ +\infty & \text { otherwise }\end{cases}
    $}
\end{equation}
The formulation given in Equation~\ref{eq:admm} is then decomposed into two sub-problems through an augmented Lagrangian method \cite{boyd_distributed_2010}, which are solved iteratively in the final concurrent framework. 
The robustness to adversarial attacks has been measured with PGD, Carlini-Wagner, and Transfer attacks \cite{madry_towards_2019, carlini_wagner, demontis_why}.

\myparagraph{HYDRA.} The final of the three selected methods, proposed in \cite{sehwag_hydra_2020}, acts by letting the pruning pipeline be aware of the robustness objective through an empirical risk minimization (ERM) based framework. 
\begin{equation}\label{eq:hydra}
    \resizebox{0.5\textwidth}{!}{$
            \hat{m}=\underset{m \in\{0,1\}^N}{\operatorname{argmin}} \underset{(x, y) \sim \mathcal{D}}{E}\left[L_{\text {pruning }}\left(\theta_{\text {pretrain }} \odot m, x, y\right)\right] \quad \text { s.t. }\|m\|_0 \leq k
    $}
\end{equation}
The HYDRA formulation in Equation~\ref{eq:hydra}, shows the search for a weight mask $\hat{m}$ which minimizes the ERM formulation of the problem, where $L_{pruning}$ can be chosen to be any other kind of loss of interest ($L_{adv}$ in the adversarial case). Given the binary nature of the mask, the network is initialized with a set of importance scores (one per weight) which are then optimized as per Equation~\ref{eq:hydra}. HYDRA marks the most accurately developed robustness evaluation, where both empirical robust accuracy, through PGD, and verifiable robust accuracy, through MixTrain and CROWNIBP, are measured \cite{madry_towards_2019, https://doi.org/10.48550/arxiv.1811.02625, https://doi.org/10.48550/arxiv.1906.06316}. Also, we reckon the authors had a WideResNet-28-10 on the unified robustness benchmark RobustBench \cite{croce2021robustbench} and briefly mentioned the analysis with the attack ensemble framework AutoAttack \cite{croce_autoattack}. Yet, not every model has been uniformly evaluated with such criteria, let alone each and every one of those presented in the paper.
